Deep Frequency-Aware Functional Maps for Robust Shape Matching

Deep functional map frameworks are widely employed for 3D shape matching. However, most existing deep functional map methods cannot adaptively capture important frequency information for functional map estimation in specific matching scenarios, i.e., lacking \textit{frequency awareness}, resulting in poor performance when dealing with large deformable shape matching. To this end, we propose a novel unsupervised learning-based framework called Deep Frequency-Aware Functional Maps, which can gracefully cope with various shape matching scenarios. We first introduce a general constraint called Spectral Filter Operator Preservation to compute desirable functional maps, where the spectral filter operator encodes informative frequency information and can promote frequency awareness for deep functional map frameworks by learning a set of filter functions. Then, we directly utilize the proposed constraint as a loss function to supervise functional maps, pointwise maps, and filter functions simultaneously, where the filter functions are derived from the orthonormal Jacobi basis, and the coefficients of the basis are learnable parameters. Finally, we develop an effective refinement strategy to improve the final pointwise map, which incorporates our constraint and learned filter functions, leading to more robust and accurate correspondences during the inference process. Extensive experimental results on various datasets demonstrate that our approach outperforms the existing state-of-the-art methods, especially in challenging settings like datasets with non-isometric deformation and inconsistent topology.

==> sec/10_bio.tex <==
\section{Biography Section}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{FeifanLuo.jpg}}]{Feifan Luo} is a Ph.D candidate at the College of Computer Science and Technology, Zhejiang University, China, supervised by professor Hongyang Chen. His research interests include geometric processing and graph representation learning. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{QinsongLi.jpg}}]{Qinsong Li} is a lecturer at the Big Data Institute, Central South University. He received his BS, MS, and PhD degrees from the School of Mathematics and Statistics of Central South University in 2015, 2018, and 2022, respectively. His research interests include geometric processing, 3D vision, and medical image computing. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{LingHu.jpg}}]{Ling Hu} is a lecturer in the School of Mathematics and Statistics at Hunan First Normal University, China. She received Ph.D. at the Central South University of China in 2019. Her research interests include geometric modeling, computer graphics, and computer-aided geometric design. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{HaiboWang.jpg}}]{Haibo Wang} 
	received the bachelor and master degrees from the Jishou University and Central South University in 2019 and 2022, respectively. He is currently pursuing his Ph.D. degree at the School of Mathematics and Statistics, Central South University, China. His research interests include geometric processing, computer-aided geometric design and 3D vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Xuhaojun.png}}]{Haojun Xu} 
	 received the bachelor and master degrees from the Langfang Normal University and North Minzu University in 2017 and 2020, respectively. He is currently pursuing his Ph.D. degree at the Schoool of Mathematics and Statistics, Central South University, China. His research interests include geometric processing, computer-aided geometric design and 3D vision
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{XinruLiu.jpg}}]{Xinru Liu} is an associate professor in the School of Mathematics and Statistics at Central South University, China. He received Ph.D. in applied mathematics and now is working on computer-aided geometric design, numerical optimization, and data mining. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ShengjunLiu.jpg}}]{Shengjun Liu}
is a full professor in the School of Mathematics and Statistics at Central South University, China. His research interests include geometric modeling, reverse engineering, computer graphics, and computer-aided geometric design. Liu has a DEng in computer science and technology from Zhejiang University. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{HongyangChen.jpg}}]{Hongyang Chen} received the Ph.D. degree from The University of Tokyo, Tokyo, Japan, in 2011. His research interests include data-driven intelligent systems, graph machine learning, big data mining, and intelligent computing. He is an adjunct professor with Hangzhou Institute for Advanced Study, The University of Chinese Academy of Sciences, and Zhejiang University, China. 
\end{IEEEbiography}
